Low-Rank Sinkhorn Factorization

Several recent applications of optimal transport (OT) theory to machine learning have relied on regularization, notably entropy and the Sinkhorn algorithm. Because matrix-vector products are pervasive in the Sinkhorn algorithm, several works have proposed to \textit{approximate} kernel matrices appearing in its iterations using low-rank factors. Another route lies instead in imposing low-rank constraints on the feasible set of couplings considered in OT problems, with no approximations on cost nor kernel matrices. This route was first explored by Forrow et al., 2018, who proposed an algorithm tailored for the squared Euclidean ground cost, using a proxy objective that can be solved through the machinery of regularized 2-Wasserstein barycenters. Building on this, we introduce in this work a generic approach that aims at solving, in full generality, the OT problem under low-rank constraints with arbitrary costs. Our algorithm relies on an explicit factorization of low rank couplings as a product of \textit{sub-coupling} factors linked by a common marginal; similar to an NMF approach, we alternatively updates these factors. We prove the non-asymptotic stationary convergence of this algorithm and illustrate its efficiency on benchmark experiments.

==> not_include/sec1.tex <==
\section{Gromov-Wasserstein Distance}
Let us denote $D\in\mathbb{R}^{n\times n}$ and $D'\in\mathbb{R}^{m\times m}$ two distance matrices which quantify similarity relationships between the points in respectively $\mathcal{X}$ and $\mathcal{Y}$.
The Gromov-Wasserstein (GW) distance is defined as
\begin{align}
\label{eq-GW}
    \text{GW}((a,D),(b,D'))=\min_{P\in\Pi(a,b)}\mathcal{E}_{D,D'}(P)
\end{align}
where $$\mathcal{E}_{D,D'}(P):= \sum_{i,j,i',j'}|D_{i,i'}-D_{j,j'}|^2 P_{i,j}P_{i',j'}.$$
In that case,in~\cite{peyre2016gromov} the authors show that one can can compute efficiently the GW objective as follow:
\begin{align}
\label{reformulation-GW-obejective}
  \mathcal{E}_{D,D'}(P)=\langle f(D)a,a\rangle +  \langle f(D')b,b\rangle -2\langle DPD',P\rangle
\end{align}
where  $f(x):=x^2$ is a point-wise operation. Then to solve Eq.~(\ref{eq-GW}), once again, one can apply a MD algorithm which leads to the following algorithm~(\ref{alg-mirror-descent}) initialized by $P_0=ab^T$.
% \begin{align*}
%     \text{GW}((a,D),(b,D'))=\min_{P\in\Pi(a,b)}\mathcal{E}_{D,D'}(P) - \varepsilon H(P)
% \end{align*}
% which leads to the following alogrithm:
\begin{algorithm}[H]
\SetAlgoLined
\textbf{Inputs:} $D,D',a,b,(\gamma_{\ell})_{\ell\geq 0},P$\\
\For{$\ell=0,\dots$}{
$C \gets - 4 D P D' - \frac{1}{\gamma_\ell}\log(P)$\\
$ P\gets \argmin\limits_{Q\in\Pi(a,b)} \langle Q,C\rangle - \frac{1}{\gamma_\ell} H(Q)$
  }
\KwResult{$\mathcal{E}_{D,D'}(P)$}
\caption{Mirror Descent \label{alg-mirror-descent}}
\end{algorithm}

Even if the objective~(\ref{eq-GW}) is not convex in $P$, one can obtain the non-asymptotic stationary convergence of the MD algorithm as the objective is smooth on $\Pi(a,b)$~\cite{ghadimi2013minibatch}. Indeed, by considering constant stepsizes $\gamma_\ell:=\frac{1}{2L}$, where $L:=\max\limits_{i,j,i',j'}|D_{i,i'}-D_{j,j'}|^2$ we obtain that for all $N\geq 1$,
$$\min_{1\leq \ell\leq N}\Vert \nabla_{\ell}\Vert_1 \leq \frac{4L D_0}{N}$$
where $\nabla_\ell$ is the generalized projected gradient and $D_0$ is the distance of the initial value to the optimal one. 
% \begin{rmq}
% For general loss function $\mathcal{L}$ between the two distance matrices, one can consider a stochastic version of the mirror descent under the assumption that $\mathcal{L}$ is a metric itself. Then one can approximate the random matrices.
% \end{rmq}

In the following we denote $(P^{(\ell)})_{\ell\geq 0}$ the oracle sequence of couplings obtained from Algorithm~(\ref{alg-mirror-descent}) and for all $\ell\geq 0$, we denote the oracle sequence of costs $C^{(\ell)}:= - 4 D P^{(\ell)} D'-\frac{1}{\gamma_{\ell}} \log(P^{(\ell)})$.

One may compute each iteration of the algorithm~(\ref{alg-mirror-descent}) by using Sinkhorn algorithm~(\ref{alg-sink}) with cost $C^{(\ell)}$ where each iteration can be performed in $\mathcal{O}(nm)$ algebraic operations given $C^{(\ell)}$. By denoting $K^{(\ell)}:=\exp(-\gamma_{\ell}C^{(\ell)}) $ and given $u^{(\ell)},v^{(\ell)}$ the outputs of the Sinkhorn algorithm computing $P^{(\ell+1)}=\text{Diag}(u^{(\ell)})  K^{(\ell)}  \text{Diag}(v^{(\ell)})$ requires $\mathcal{O}(n^2)$ operations. However computing $C^{(\ell)}$ and $\mathcal{E}_{D,D'}(P)$ requires in general $\mathcal{O}(nm(n+m))$ algebraic operations. Therefore this first procedure to compute the GW distance has a complexity at least cubic with respect to the number of samples at each iteration. In the following we show that if the distance matrices admits a low-rank factorization, one can obtain a linear time algorithm to compute the GW distance.
% Notice that the iterations of the Sinkhorn algorithm~(\ref{alg-sink}) are costly because of the product matrix-vector, but as soon as we have access to a positive low-rank factorization of the kernel $K$ of the form $K=V_1V_2$ where $V_1,(V_2)^{T}\in\mathbb{R}^{n\times r'}$, only $\mathcal{O}(r'n)$ operations are needed to perform each iteration of the Sinkhorn algorithm.
% In the following we denote $u,v=\text{Sinkhorn}(V_1,V_2,a,b,\delta)$ the outputs of the Sinkhorn algorithm~(\ref{alg-sink}) if such a decomposition is available.

==> not_include/sec2.tex <==
\section{Quadratic Time Approximation of the Gromov-Wasserstein Distance}
We consider the case where $n=m$ in the following for simplicity. Let us now present our main assumption on the distance matrix $D$ and $D'$. 

\begin{assumption}
\label{assump-low-rank}
Assume  that $D$ and $D'$ admit a low-rank factorization, that is there exists $A\in\mathbb{R}^{n\times r}$ and $B\in\mathbb{R}^{n\times r'}$ such that
\begin{align*}
    D = AA^{T}\quad \text{and}\quad D' = BB^{T}.
\end{align*}
\end{assumption}
In fact the above assumption can be relaxed by considering cost matrix of the form:
\begin{align*}
D =\sum_{k=1}^K A_kB_k^{T} 
\end{align*}
where for all $k\in\{1,\dots,K\}$, $A_k\in\mathbb{R}^{n\times r_k}$ and $B_k^{T}\in\mathbb{R}^{r_k\times n}$. In the following, for simplicity of the notations we will consider the case where $D$ and $D'$ are semi-positive definite. 
\begin{rmq}
Note that in the GW distance $D$ and $D'$ are always distance matrices and therefore a low-rank approximation can be obtained in linear time as discussed in Section~\ref{sec-low-rank-distance}.
% Indeed, by denoting $r_{\text{tot}}:=\sum_{k=1}^K r_k$, one can define $A_{\text{tot}}:=[A_1,...,A_K]\in\mathbb{R}^{n\times r_{\text{tot}}}$ and $B_{\text{tot}}:=[B_1,...,B_K]\in\mathbb{R}^{n\times r_{\text{tot}}}$ and obtain that $D=A_{\text{tot}}B_{\text{tot}}^T$. 
\end{rmq}

\paragraph{Computational cost.} In that case observe that for any given $P\in\mathbb{R}^{n\times m}$ and $\gamma>0$, one can compute 
\begin{align*}
    C = - 4 A A^{T} P B B^{T} - \frac{1}{\gamma}\log(P)
\end{align*}
in $\mathcal{O}(n^2 r)$ algebraic operations. Moreover thanks to the reformulation of $\mathcal{E}_{D,D'}(P)$ given in~(\ref{reformulation-GW-obejective}), one can compute it in quadratic time also. Indeed the computation of $\langle f(D) a,a\rangle$ and $\langle f(D') b,b\rangle$ can be obtained in $\mathcal{O}(n^2)$. Moreover by denoting $G:=A^TPB\in\mathbb{R}^{r\times r}$, we have
\begin{align*}
    \langle DPD',P\rangle & = \text{Tr}(GG^T).
\end{align*}
Computing $G$ given $P$ requires only $\mathcal{O}(n^2r)$ algebraic operations, and computing the square norm of $G$ needs only $\mathcal{O}(r^2)$ algebraic operations. Thus the overall complexity to compute  $\mathcal{E}_{D,D'}(P)$ is $\mathcal{O}(n^2r+r^2)$.
% Indeed by first computing $G = A^{T} P B \in\mathbb{R}^{r\times r}$ in $\mathcal{O}(n^2 r)$ algebraic operations, one obtain $C = - 4 A G B^{T}$ $K=\exp(-C/\varepsilon)$ with the same order of operations. 
% Note also that given $u,v$ the outputs of the Sinkhorn algorithm~(\ref{alg-sink}) and $K$, computing $P=\text{Diag}(u)  K  \text{Diag}(v)$ requires $\mathcal{O}(n^2)$ operations.
 % \paragraph{Efficient Computation of $\mathcal{E}_{D,D'}(P)$.} In~\cite{peyre2016gromov} the authors show that 
% \begin{align*}
%      \mathcal{E}_{D,D'}(P)= \langle f(D) a,a\rangle + \langle f(D') b,b\rangle - 2 \langle DPD',P\rangle 
% \end{align*}
% where  $f(x):=x^2$ is a point-wise operation. 
% As $D$ and $D'$ admits a low-rank factorization by assumption, the computation of $\langle f(D) a,a\rangle$ and $\langle f(D') a,a\rangle$ can be obtained in linear time with respect to the number of samples. Indeed, remark that for $x,y\in\mathbb{R}^r$,
% $$\langle x,y\rangle^2=\sum_{i,j=1}^r x_ix_j y_iy_j $$
% Therefore by denoting $\mathcal{A}:=\{a_1,...a_n\}$ the rows of the matrix $A$ and $\psi(x):= \text{Vect}(xx^T)\in\mathbb{R}^{r^2}$ where $\text{Vect}(\cdot)$ is the vectorization operation, we obtain that
% \begin{align*}
%     f(D)=\tilde{A}\tilde{A}^T \text{\quad where}\\
%   \tilde{A}^T = [\psi(a_1),\dots,\psi(a_n)]\in\mathbb{R}^{r^2\times n}
% \end{align*}
% Therefore we have
% \begin{align*}
%   \langle f(D) a,a\rangle =   \langle \tilde{A}^T  a, \tilde{A}^T a\rangle 
% \end{align*}
% which can be performed in $\mathcal{O}(nr^2)$ given $\tilde{A}$. \todo{linear approx of the first constant: should we put it here or in the linear section ?}
% First note that the computation of $\langle f(D) a,a\rangle$ and $\langle f(D') b,b\rangle$ can be obtained in quadratic time with respect to the number of samples. Moreover we have that 
% \begin{align*}
%     \langle DPD',P\rangle & = \text{Tr}(P^TAA^TPBB^T)\\
%      &= Tr(GG^T)
% \end{align*}
% Recall that computing $ G\in\mathbb{R}^{r\times r}$ given $P$ requires only $\mathcal{O}(n^2r)$ algebraic operations, and therefore computing the square norm of $G$ needs only $\mathcal{O}(r^3)$ algebraic operations. Finally the overall complexity to compute  $\mathcal{E}_{D,D'}(P)$ is $\mathcal{O}(n^2r+r^3)$.
Let us now introduce the following algorithm initialized with $P_0:=ab^T$:
\begin{algorithm}[H]
\SetAlgoLined
\textbf{Inputs:} $D,D',a,b, I, (\gamma_{\ell})_{0 \leq \ell\leq I-1},(\mu_{\ell})_{0 \leq \ell\leq I-1}$, P\\
\For{$\ell=0,\dots,I-1$}{
$G \gets A^{T} P B$\\
$C \gets 4 A G B^{T}-\frac{1}{\gamma_\ell}\log(P)$, $K \gets \exp(- \gamma_\ell C)$ \\
$u,v = \text{Sinkhorn}(K,a,b,\mu_{\ell}) \quad \text{(Algorithm~(\ref{alg-sink}))}$\\
$P = \text{Diag}(u)  K  \text{Diag}(v)$
  }
\KwResult{$\mathcal{E}_{D,D'}(P)$}
\caption{Quadratic-GW \label{alg-quad-GW}}
\end{algorithm}
Finally the overall computation of the Algorithm~(\ref{alg-quad-GW}) costs $\mathcal{O}(n^2 (Ir + T)+ nr^2)$ algebraic operations where $T=\sum_{\ell=0}^ {I-1}T_\ell$ and $T_\ell$ is the number of iterations of the Sinkhorn algorithm~(\ref{alg-sink}) at iteration $\ell$ for a precision $\mu_\ell$. 
\todo{add the error of Sinkhorn in the study of stationary point?}
% \begin{rmq}
% Let $I\geq 1$ and $\delta>0$. In theorem~\ref{thm:quadratic-GW}, we show that for well chosen $(\mu_{\ell})_{0 \leq \ell\leq I-1}$, the Quadratric-GW Algorthm~(\ref{alg-quad-GW}) with input $P^{(0)}$ outputs an approximation of the GW distance $\widehat{\mathcal{E}}$ and a coupling $\widehat{P}$ such that:
% \begin{align*}
%     \Vert P^{(I)} - \widehat{P}\Vert_1&\leq \frac{\delta}{2L}\\
%     |\mathcal{E}_{D,D'}(P^{(I)}) - \widehat{\mathcal{E}}|&\leq \delta
% \end{align*}
% in $\mathcal{O}(n^2 (Ir + T)+ nr^2 + r^3 )$ algebraic operations where
%  $T\in \tilde{\mathcal{O}}\left(I\left(\frac{LIR^I}{\varepsilon^I\delta}\right)^2\right)$, $L:=\sup_{i,j,k,l}|D_{i,k}-D_{j,j}|^2$, $R:=4 \Vert D\Vert_{\text{op}}\Vert D'\Vert_{\text{op}}$ and the notation $\tilde{\mathcal{O}}(.)$ means that we omits polylogarithmic factors w.r.t the constants of the problem. See proof in Appendix~\ref{sec:quad-GW}.
% \end{rmq}

From the Assumption~(\ref{assump-low-rank}) one can in fact accelerate the computation of the GW distance and obtain a linear time algorithm with respect to the number of samples thanks to the ideas presented in Section~\ref{sec-OT-linear}. In the following we present two methods where the first one aims to directly obtain a positive low-rank approximation of the coupling at each iteration and the second one uses a positive factorization of the kernel at each iteration.



==> not_include/sec3.tex <==
\section{Positive Low-rank Approximation of the Transport Plan}
As in the classical OT problem, we can constraint the coupling of the GW distance to have a low non-negative rank. In the following we present two algorithms which have a linear time complexity where either the marginal $g$ is fixed or not.


\subsection{The Fixed Marginal Case}
Let $r\geq 1$, $g\in\Delta_r^{*}$ and let us consider the following objective:
\begin{align}
\label{eq-LRGW-fixed}
    \text{GW}_{r}((a,D),(b,D'))=\min_{P\in\Pi_{a,g,b}}\mathcal{E}_{D,D'}(P)
\end{align}
which can be formulated as follows:
\begin{align*}
  \text{GW}_{r}((a,D),(b,D'))=  \min_{(Q,R)\in\Pi_{a,g}\times\Pi_{b,g}}\mathcal{E}_{D,D'}(Q,R)
\end{align*}
where 
\begin{align*}
    \mathcal{E}_{D,D'}(Q,R):= &\sum_{i,j,i',j'}|D_{i,i'}-D_{j,j'}|^2\\ &[Q\text{Diag}(1/g)R^T]_{i,j}[Q\text{Diag}(1/g)R^T]_{i',j'}.
\end{align*}
Applying a MD algorithm to the above objective leads for all $\ell\geq 0$ to the following updates:
\begin{align*}
    Q^{(\ell+1)}&:=\argmin_{Q\in\Pi_{a,g}}\langle C^{(\ell)}_{1},Q\rangle -\frac{1}{\gamma_\ell}H(Q)\\
        R^{(\ell+1)}&:=\argmin_{R\in\Pi_{a,g}}\langle C^{(\ell)}_{2} ,R\rangle -\frac{1}{\gamma_\ell}H(R)
\end{align*}
where $(Q_0,R_0)\in\Pi_{a,g}\times\Pi_{b,g}$ is an initial point, $C^{(\ell)}_{1}:=\widetilde{C}^{(\ell)}R^{(\ell)}\text{Diag}(1/g)-\frac{1}{\gamma_\ell}\log(Q^{(\ell)})$,  $ C^{(\ell)}_{2}:=(\widetilde{C}^{(\ell)})^TQ^{(\ell)}\text{Diag}(1/g)-\frac{1}{\gamma_\ell}\log(R^{(\ell)})$, $\widetilde{C}^{(\ell)}:= - 4 A A^{T} P^{(\ell)} B B^{T}$, $P^{(\ell)}:=Q^{(\ell)}\text{Diag}(1/g)(R^{(\ell)})^T$ and $\gamma_\ell$ is a sequence of positive real numbers. 

To obtain the non-asymptotic convergence of the MD algorithm, we show in the following proposition that $\mathcal{E}_{D,D'}(Q,R)$ is a smooth function.
\begin{prop}
The function $(Q,R)\rightarrow \mathcal{E}_{D,D'}(Q,R)$ is differentiable on $\mathbb{R}^{n\times r}\times \mathbb{R}^{n\times r}$ 
and for any $X,Y\in \Pi_{a,g}\times\Pi_{b,g}$, we have
\begin{align*}
\Vert \nabla \mathcal{E}_{D,D'}(X) - \nabla \mathcal{E}_{D,D'}(Y)\Vert_{*}\leq& 8\Vert 1/g\Vert_{\infty} L(r+1)\\
&\Vert X-Y\Vert 
\end{align*}
where $L:=\max\limits_{i,j,i',j'}|D_{i,i'}-D_{j,j'}|^2$, $\Vert(Q,R)\Vert=\max(\Vert Q\Vert_1,\Vert R\Vert_1)$ and its dual norm is $\Vert (Q,R)\Vert_{*}:=\Vert Q\Vert_{\infty}+\Vert R\Vert_{\infty}$.
\end{prop}
\begin{proof}
$\mathcal{E}_{D,D'}(Q,R)$ is clearly differentiable. By denoting $\mathcal{L}(\cdot):=(|D_{i,i'}-D_{j,j'}|^2)_{i,i',j,j'}$ the linear operator on $\mathbb{R}^{n\times n}$, $X:=(Q,R)\in\mathbb{R}^{n\times r}\times \mathbb{R}^{n\times r}$ and $P:=Q\text{Diag}(1/g)R^T$, we have that:
\begin{align*}
\nabla\mathcal{E}_{D,D'}(X)=       
            \begin{pmatrix}
           2\mathcal{L}(P)R\text{Diag}(1/g)\\           
           2\mathcal{L}(P)^T Q\text{Diag}(1/g) 
    \end{pmatrix}    
\end{align*}
Therefore we have for any $(Q_1,R_1),~(Q_2,R_2)\in\Pi_{a,g}\times\Pi_{b,g}$ that
\begin{align*}
 &\Vert \nabla\mathcal{E}_{D,D'}(Q_1,R_1) - \nabla\mathcal{E}_{D,D'}(Q_2,R_2)\Vert_{*}\\
 &=\Vert 2\mathcal{L}(P_1)R_1\text{Diag}(1/g) - 2\mathcal{L}(P_2)R_2\text{Diag}(1/g)\Vert_{\infty}\\
 &+\Vert 2\mathcal{L}(P_1)^T Q_1\text{Diag}(1/g) - 2\mathcal{L}(P_2)^T Q_2\text{Diag}(1/g) \Vert_{\infty}.
\end{align*}
Moreover we have
\begin{align*}
    &\Vert 2\mathcal{L}(P_1)R_1\text{Diag}(1/g) - 2\mathcal{L}(P_2)R_2\text{Diag}(1/g)\Vert_{\infty}\\
    &\leq 2 \Vert\text{Diag}(1/g)\Vert_{\infty} (\Vert (\mathcal{L}(P_1) - \mathcal{L}(P_2))R_1\Vert_\infty\\
    &+ \Vert \mathcal{L}(P_2) (R_1 - R_2)\Vert_\infty)\\
    &\leq 2 \Vert\text{Diag}(1/g)\Vert_{\infty} L (\Vert P_1 - P_1\Vert_{1} + \Vert R_1 - R_2\Vert_1).
\end{align*}
Remark that 
\begin{align*}
    \Vert P_1 - P_1\Vert_{1} &\leq \Vert (Q_1-Q_2)\text{Diag}(1/g)R_1^{T}\Vert_1\\
    &+\Vert Q_2(\text{Diag}(1/g)R_1^{T}-\text{Diag}(1/g)R_2^{T})\Vert_1\\
    &\leq r( \Vert Q_1 - Q_2\Vert_1 +\Vert R_1 - R_2\Vert_1)
\end{align*}
Therefore we obtain that 
\begin{align*}
     &\Vert 2\mathcal{L}(P_1)R_1\text{Diag}(1/g) - 2\mathcal{L}(P_2)R_2\text{Diag}(1/g)\Vert_{\infty}\\
    &\leq 2 \Vert\text{Diag}(1/g)\Vert_{\infty} L(r+1) (\Vert Q_1 - Q_2\Vert_1  + \Vert R_1 - R_2\Vert_1)\\
    &\leq 4 \Vert\text{Diag}(1/g)\Vert_{\infty} L(r+1)\Vert (Q_1-Q_2,R_1-R_2)\Vert
\end{align*}
An analogue proof leads to the same upper bound for the second term $\Vert 2\mathcal{L}(P_1)^T Q_1\text{Diag}(1/g) - 2\mathcal{L}(P_2)^T Q_2\text{Diag}(1/g) \Vert_{\infty}$ involved in the norm of the diffence of the two gradients which gives that $\mathcal{E}_{D,D'}$ is $L_{\text{LR}}:=8\Vert\text{Diag}(1/g)\Vert_{\infty} L(r+1)$-smooth according to the $\ell_1$ norm.
\end{proof}

As the objective is smooth with respect to the norm $\Vert(Q,R)\Vert:=\max(\Vert Q\Vert_1, \Vert R\Vert_1$), we obtain the non-asymptotic convergence of the MD algorithm.

\subsection{The Free Marginal Case}

% \paragraph{Computing the Cost Matrix.} Observe that for any given $P\in\mathbb{R}^{n\times m}$, one can compute 
% \begin{align*}
%     C = -  A A^{T} P B B^{T}
% \end{align*}
% in $\mathcal{O}(n^2 r)$ algebraic operations. Indeed by first computing $G = A^{T} P B \in\mathbb{R}^{r\times r}$ in $\mathcal{O}(n^2 r)$ algebraic operations, one obtain $C = - A G B^{T}$ with the same order of operations. Moreover if the matrix $P$ admits a low-rank factorization such that $P:=QR^{T}$ where $Q,R\in\mathbb{R}^{n\times r_{\ell}}$, then computing $C$ cost only $\mathcal{O}(r(r_{\ell}+r)n)$ algebraic operations. Therefore given $P^{(\ell)}$, one can obtain $C^{(\ell)}$ in quadratic time with respect to the number of samples, and if $P^{(\ell)}$ admits a low-rank factorization then the computation of $C^{(\ell)}$ becomes linear.

% The remaining question is to determine the cost of obtaining $P^{(\ell+1)}$ from the cost matrix $C^{(\ell)}$. Indeed $P^{(\ell+1)}$ is obtained by solving 
% \begin{align*}
%       P^{(\ell+1)} &= \min_{P\in\Pi(a,b)} \langle R,C^{(\ell)}\rangle - \varepsilon H(P)\quad
% \end{align*}
% By denoting $K^{(\ell)}:=\exp(-C^{(\ell)}/\varepsilon)$ which can be computed in $\mathcal{O}(n^2)$ algebraic operations from $C^{(\ell)}$, one can apply the Sinkhorn iterations and obtained $P^{(\ell+1)}$ in quadratic time also if we do not consider the dependence in $\varepsilon$. Overall each iteration of the GW algorithm is quadratic in time if we do not consider the dependence in $\varepsilon$. 

% In fact we can do even better by looking directly for a low-rank coupling.



\section{Positive Factorization of the Kernel}


\begin{algorithm}[H]
\SetAlgoLined
\textbf{Inputs:} $A,B,R,r$\\
 $V_1 \gets \varphi(-A^T)^T$,$\quad V_2 \gets \varphi(B^T)$\\
\textbf{Result:} $V_1,V_2$
\caption{$\text{RF-Approx}(A,B,R,r)$ \label{alg-rf-approx}}
\end{algorithm}


Here we consider a regularized version of the GW distance introduced in~\cite{peyre2016gromov} defined as follows:
\begin{align*}
    \min_{P\in\Pi(a,b)}\mathcal{E}_{D,D'}(P) - \varepsilon H(P)
\end{align*}

Instead of computing the whole matrix $C^{(\ell)}$, we may instead obtain a positive factorization of the kernel $K^{(\ell)}$ associated. Let us assume for now that $P^{(\ell)}$ admits a low rank factorization of the form $P^{(\ell)}=P_1^{(\ell)}P_2^{(\ell)}$ where $P_1^{(\ell)},(P_2^{(\ell)})^T\in\mathbb{R}^{n\times r_{\ell}}$ and $r_\ell\in\mathbb{N}_{*}$. We will show in the following that if $P^{(\ell)}$ admits such a decomposition, then $P^{(\ell+1)}$ admits also a low-rank factorization and therefore under a well-suited initialization, then the algorithm produces low-rank couplings. Indeed, under assumption~(\ref{assump-low-rank}), remark that we have
\begin{align*}
    C^{(\ell)} &= - T^{(\ell)}U^{(\ell)} \quad~\text{where}\\
    T^{(\ell)} &= 4A\in\mathbb{R}^{n\times r} \\
    U^{(\ell)} &=G^{\ell} B^{T} \in \mathbb{R}^{r\times n}  \\
    G^{(\ell)} &= A^{T} P^{(\ell)} B \in \mathbb{R}^{r\times r}
\end{align*}
Here we do not compute explicitly  $C^{(\ell)}$ but simply $T^{(\ell)}$ (which is constant through the iterations of the algorithm) and $U^{(\ell)}$ which can be obtained in $\mathcal{O}(rn (r+ r_{\ell}))$ operations thanks to the low-rank factorization of $P^{(\ell)}$. In that case the matrix  $K^{(\ell)}=\exp(-\gamma_{\ell}C^{(\ell)})$ can be approximated by a positive low rank factorization in linear time with respect to the number of samples. Indeed we have that 
\begin{align*}
 K^{(\ell)}=\exp(\gamma_{\ell} T^{(\ell)}U^{(\ell)})\odot P^{(\ell)}
\end{align*}
Note first that one can obtain a positive low-rank approximation of the kernel $K_1^{(\ell)}:=\exp(\gamma_{\ell} T^{(\ell)}U^{(\ell)})$ of the form $\widehat{K_1}^{(\ell)}= $ as discussed in Section~\ref{sec-positive-kernel-OT} 


 In that case one can also recover a factorization of $\tilde{K}$, as one can always rewrite $\tilde{K}$ which is of the form $AB\odot CD$ as $\tilde{A}\tilde{B}$ by considering the following equality 
$\langle x_i,y_j\rangle \times \langle x_i',y_j'\rangle = \sum_{k,l}[x_i]_k[x_i']_l [y_j]_k[y_j']_l=\langle \phi(x_i,x_i'),\phi(y_j,y_j')\rangle$. See paper convergence of mirror descent non convex.

% \paragraph{Low-rank Approximation of Dot-product Kernels.} Considering the analytic formulation of the exponential function leads to a decent feature maps from which a low rank approximation of the kernel of the form $\widetilde{K}^{(\ell)}=V_1^{(\ell)} V_2^{(\ell)}$ is obtained where  $V_1^{(\ell)}\in\mathbb{R}^{n\times r_{\ell}}$ and $V_2^{(\ell)}\in\mathbb{R}^{r_{\ell}\times n}$. Now one may want to ensure that the coefficients of the new kernel matrix obtained are all positives as in~\cite{altschuler2020polynomialtime}. The main interest of using such technique is to exploit the polynomial structure of the approximation which leads to faster algorithm as soon as $r$ times the degree of the polynomial approximation of the exponential function is lower than $r_{\ell}$. Indeed by considering instead a decomposition of the cost function as the following:
% \begin{align*}
% D =\sum_{k=1}^r A_kB_k^{T}     
% \end{align*}
% where $A_k,B_k\in\mathbb{R}^{n}$, the cost per iteration of the Sinkhorn algorithm becomes $\mathcal{O}(rd\times n)$.


% \paragraph{Nystrom method.} By denoting $X^{(\ell)}:=[(T^{(\ell)})^{T},(U^{(\ell)})]^T\in\mathbb{R}^{2n\times r}$, one remarks that $K^{(\ell)}$ is just the upper right sub matrix of the matrix $\widehat{K}^{(\ell)}:=\exp(X^{(\ell)}(X^{(\ell)})^T/\varepsilon)\in\mathbb{R}^{2n\times 2n}$ which is symmetric positive semi-definite. One can therefore obtain a low rank approximation of $\widehat{K}^{(\ell)}$ in linear time with respect to the number of samples thanks to the Nystrom method. Indeed let us denote
% $X_{r_{\ell}}^{(\ell)}:=(\widehat{x}_1^{(\ell)},...,\widehat{x}_{r_{\ell}}^{(\ell)})^T$ a subset of $r_{\ell}$ rows in $X^{(\ell)}:=(x_1^{(\ell)},...,x_{2n}^{(\ell)})^T$. One can construct an approximation of
% $\widehat{K}^{(\ell)}$ by considering a matrix $V^{(\ell)}\in\mathbb{R}^{2n\times r_{\ell}}$ defined as
% $[V_1^{(\ell)}]_{ij}:=\exp(\langle x_i^{(\ell)},\widehat{x}_j^{(\ell)}\rangle/\varepsilon)$, a
% matrix $V_2^{(\ell)}=(V_1^{(\ell)})^T$  and a matrix $M^{(\ell)}\in\mathbb{R}^{r_{\ell}\times r_{\ell}}$ defined as $M^{(\ell)}_{jj'}:=\exp(\langle \widehat{x}_i^{(\ell)},\widehat{x}_j^{(\ell)}\rangle/\varepsilon)$ such that 
% $\widetilde{K}^{(\ell)}= V_1^{(\ell)} (M^{(\ell)})^{-1}V^{(\ell)}_2$.  Note that this factorization can be forced to have positive coefficients~\cite{altschuler2018massively} which guarantee the convergence of the Sinkhorn algorithm.

% The main issue with the two above techniques are that they require an extreme precision to guarantee that the entries of the approximated kernel are positive. Indeed as soon as there exists one negative entry in the kernel matrix, the Sinkhorn algorithm fails to converge. In the specific case of the GW distance, one has to repeat the Sinkhorn algorithm~(\ref{alg-sink}) multiple times, therefore it is very unlikely that these two above methods converge with a reasonable $r_{\ell}$. In the following we present another way of obtaining such approximation while guarantying the positivity of the entries of the kernel matrix obtained. Indeed by construction, the Sinkhorn algorithm~(\ref{alg-sink}) will always converge by using such technique whatever the precision asked for the approximation.



% \paragraph{Positive Random Features.} By denoting
% $\mathcal{T}:=\{t_1^{(\ell)},\cdots,t_n^{(\ell)}\}$ and $\mathcal{U}:=\{u_1^{(\ell)},\cdots,u_n^{(\ell)} \}$ respectively the set of columns of $(T^{(\ell)})^T$ and $U^{(\ell)}$, we remark that for all $i,j\in\{1,...,n\}$, $K^{(\ell)}_{ij}=\exp(\langle t_i^{(\ell)}, u_j^{(\ell)}\rangle/\varepsilon)$. In~\cite{scetbon2020linear}, the authors manage to obtain a positive factorization of the Gaussian kernel from which they deduce a uniform control of the ratio when approximating such kernel. Because they manage to control the ratio instead of the difference between the Gaussian kernel and its approximation we can deduce directly from their results a ratio control for the following dot-product kernel  $k(t,u):=\exp(\langle t, u\rangle/\varepsilon)$. More precisely, let $R_{\ell}:=\max\limits_{1\leq i\leq n}\max\left(\Vert u_i^{(\ell)}\Vert_2,\Vert t_i^{(\ell)}\Vert_2 \right)$, $q_{\ell}=\frac{R_{\ell}^2}{4\varepsilon r W_0\left(R_{\ell}^2/ (2 \varepsilon r)\right)}$ where $W_0$ is the Lambert function, $\sigma^2_{\ell} =q_{\ell}\varepsilon/2$, $\rho_{\ell}=\mathcal{N}\left(0,\sigma^2_{\ell}\text{I}_r\right)$ and let us define for all $t,x\in\mathbb{R}^r$ the following map
% \begin{align*}
%     \varphi_{\ell}(t,x)&=(2q_{\ell})^{d/4}\exp\left(\frac{\Vert t\Vert_2^2}{2\varepsilon}\right)\\
%     &\exp\left(-\varepsilon^{-1} \Vert t-x\Vert^2_2\right)\exp\left(\frac{\varepsilon^{-1}\Vert x\Vert_2^2}{2q_{\ell}}\right)
% \end{align*}
% Then for any $t,u\in\mathbb{R}^r$, \cite{scetbon2020linear} show that 
% $$k(t,u)=\int_{x\in\mathbb{R}^d} \varphi_{\ell}(t,x)\varphi_{\ell}(u,x) d\rho(x)$$
% and that
% \begin{align*}
% \psi_{\ell}:=\sup_{t,u\in \mathcal{B}(0,R_{\ell})}\sup_{x\in\mathbb{R}^r}\left|\frac{\varphi(t,x)\varphi(y,u)}{k(u,x)}\right|<+\infty
% \end{align*}
% Let $r_{\ell}\geq 1$, $x_1,...,x_{r_{\ell}}\in\mathbb{R}^{r}$, and let us denote  
% $$\varphi_{\ell}(t):=\frac{1}{\sqrt{r_{\ell}}}\left(\varphi(t,x_1),...,\varphi(t,x_{r_{\ell}})\right)\in\mathbb{R}^{r_{\ell}}.$$ 
% and 
% $$ k_{\ell}(t,u):=\langle \varphi_{\ell}(x),\varphi_{\ell}(y)\rangle.$$ 
% Then in~\cite{scetbon2020linear} the authors show that if $x_1,...,x_{r_{\ell}}$ are drawn independently from $\rho_{\ell}$ we have that
% \begin{align*}
% \mathbb{P}\left(\sup_{(t,u)\in \mathcal{T}\times\mathcal{U}}\left |\frac{k_{\ell}(x,y)}{k(x,y)}-1\right|\geq \delta\right)\leq 2 n^2\exp\left(-\frac{r \delta^2}{2 \psi_{\ell}^2}\right)
% \end{align*}
% Therefore by denoting $V_1^{(\ell)}:=[\varphi_{\ell}(t_1^{(\ell)}),\dots,\varphi_{\ell}(t_n^{(\ell)})]^{T}\in\mathbb{R}^{n\times r_{\ell}}$ and $V_2^{(\ell)}:=[\varphi_{\ell}(u_1^{(\ell)}),\dots,\varphi_{\ell}(u_n^{(\ell)})]\in\mathbb{R}^{r_{\ell}\times n}$, we can obtain an approximation of the kernel matrix $K^{(\ell)}$ as follows
% $\widetilde{K}^{(\ell)}:= V_1^{(\ell)} V_2^{(\ell)}.$
% Note that computing $V_1^{(\ell)}$ and  $V_2^{(\ell)}$ cost only $\mathcal{O}(nrr_{\ell})$ algebraic operations. Therefore this method allows to obtain a positive factorization of $K^{(\ell)}$ in linear time with respect to the number of samples.
% \begin{algorithm}[H]
% \SetAlgoLined
% \textbf{Inputs:} $T,U,R_\ell,r_{\ell}$\\
%  $V_1 \gets \varphi_{\ell}(T^T)$,$\quad V_2 \gets \varphi_{\ell}(U)$\\
% \textbf{Result:} $V_1,V_2$
% \caption{$\text{RF-Approx}(T,U,R_\ell,r_{\ell})$ \label{alg-rf-approx}}
% \end{algorithm}

% In Algorithm~(\ref{alg-rf-approx}), the operation $\varphi_{\ell}(\cdot)$ has to be understood as a column-wise operation. Moreover, once $V_1^{(\ell)}$ and  $V_2^{(\ell)}$ are computed, each iteration of the Sinkhorn algorithm~(\ref{alg-sink}) costs only $\mathcal{O}(r_{\ell}n)$ algebraic iterations. 



\paragraph{Efficient Computation of $G^{(\ell+1)}$.} The final step remains in computing $P^{(\ell+1)}$ from the output $u^{(\ell+1)}$ and $v^{(\ell+1)}$ of the Sinkhorn algorithm. In fact we do not even need to compute this matrix as we can simply keep its factorized formulation given by:
\begin{align*}
    P^{(\ell+1)}= \text{Diag}(u^{(\ell+1)})  V_1^{(\ell)} V^{(\ell)}_2 \text{Diag}(v^{(\ell+1)})
\end{align*}
Therefore $G^{(\ell+1)}$ can be computed in $\mathcal{O}(r r_{\ell} n)$. Indeed we have:
\begin{align*}
     G^{(\ell+1)} &= A^{T} P^{(\ell+1)} B \\
 &=  G_1^{(\ell+1)} G_2^{(\ell+1)} 
\end{align*}
where 
\begin{align*}
 G_1^{(\ell+1)}&:=A^{T} \text{Diag}(u^{(\ell+1)})  V_1^{(\ell)} \\
 G_2^{(\ell+1)}&:=V^{(\ell)}_2 \text{Diag}(v^{(\ell+1)}) B   
\end{align*}
Computing $G_1^{(\ell+1)}$ can be done in $\mathcal{O}(rr_{\ell}n)$. Indeed by first computing $\widehat{G}_1^{(\ell+1)}:=A^{T} \text{Diag}(u^{(\ell+1)})\in\mathbb{R}^{r\times n}$ which has a cost of $\mathcal{O}(rn)$ algebraic operations, we obtain $G_1^{(\ell+1)}=\widehat{G}_1^{(\ell+1)}V^{(\ell)}_1$ in $\mathcal{O}(rr_{\ell}n)$ operations. It is the same for $G_2^{(\ell+1)}$ which leads to a total cost of $\mathcal{O}(rr_{\ell}n)$ to compute $G^{(\ell+1)}$.

% \begin{rmq}
% Note that when $\widetilde{K}^{(\ell)}=V_1^{(\ell)} V_2^{(\ell)}$, it is exactly the same case as before where $M^{(\ell)}=I_{r_{\ell}}$.
% \end{rmq}

\paragraph{Efficient Computation of $\mathcal{E}_{D,D'}(P)$.} Recall that we have 
\begin{align*}
     \mathcal{E}_{D,D'}(P):= \langle f(D) a,a\rangle + \langle f(D') a,a\rangle - 2 \langle DPD',P\rangle 
\end{align*}
where  $f(x):=x^2$ is a point-wise operation. As $D$ and $D'$ admits a low-rank factorization by assumption, the computation of $\langle D a,a\rangle$ and $\langle D' a,a\rangle$ can be obtained in $\mathcal{O}(nr^2)$ operations. Indeed, remark that for $x,y\in\mathbb{R}^r$,
$$\langle x,y\rangle^2=\sum_{i,j=1}^r x_ix_j y_iy_j $$
Therefore by denoting $\mathcal{A}:=\{a_1,...a_n\}$ the rows of the matrix $A$ and $\psi(x):= \text{Vect}(xx^T)\in\mathbb{R}^{r^2}$ where $\text{Vect}(\cdot)$ is the vectorization operation, we obtain that
\begin{align*}
    f(D)=\tilde{A}\tilde{A}^T \text{\quad where}\\
   \tilde{A}^T = [\psi(a_1),\dots,\psi(a_n)]
\end{align*}
Therefore we have
\begin{align*}
  \langle f(D) a,a\rangle =   \langle \tilde{A}^T  a, \tilde{A}^T a\rangle 
\end{align*}
which can be performed in $\mathcal{O}(nr)$ given $\tilde{A}$. Also note that the computation of $\tilde{A}^T$ requires also $\mathcal{O}(nr^2)$ given $A$. Moreover we have that 
\begin{align*}
    \langle DPD',P\rangle &= \text{Tr}(P^TAA^TPBB^T)\\
    &= Tr(G^{(\ell+1)}(G^{(\ell+1)})^T)
\end{align*}
Recall that computing $ G^{(\ell+1)}\in\mathbb{R}^{r\times r}$ requires only $\mathcal{O}(rr_{\ell}n)$ algebraic operations, and therefore computing the trace of the product by itself needs only $\mathcal{O}(r^3)$ algebraic operations. Finally the overall computation cost to obtain the GW distance at iteration $\ell$ given the factorization of $P^{(\ell)}$ is $\mathcal{O}(nr(r_{\ell}+r)+r^3)$.

Let us now introduce our first algorithm to compute the GW distance.
\begin{algorithm}[H]
\SetAlgoLined
\textbf{Inputs:} $A,B,u,v,V_1,V_2,a,b,I, (R_{\ell})_{ 0 \leq \ell\leq I-1},\\
(r_{\ell})_{ 0 \leq \ell\leq I-1},(\mu_{\ell})_{ 0 \leq \ell\leq I-1}$\\
\For{$\ell=0,\dots,I-1$}{
$G_1 \gets A^{T} \text{Diag}(u) V_1$, $G_2 \gets V_2 \text{Diag}(v) B$ \\
$G \gets G_1 G_2$, $U=G B^{T}$\\
$V_1,V_2 \gets \text{RF-Approx}(4A,U,R_{\ell},r_{\ell})$ (Algorithm~(\ref{alg-rf-approx}))\\
$ u,v \gets \text{Sinkhorn}(V_1,V_2,a,b,\mu_{\ell})$ (Algorithm~(\ref{alg-sink}))
  }
$G_1 \gets A^{T} \text{Diag}(u) V_1$, $G_2\gets V_2 \text{Diag}(v) B$ \\
$G \gets G_1 G_2$, $M\gets G G^{T}$\\
$c \gets \Vert A^Ta\Vert_2^2 + \Vert B^Tb\Vert_2^2$\\
$\mathcal{E}\gets c - 2\text{Tr}(M)$ \\
\textbf{Result:} $\mathcal{E}$
\caption{RF-LinearGW \label{alg-lin-GW}}
\end{algorithm}

In the Algorithm~(\ref{alg-lin-GW}), we initialize $P^{(0)}:=\text{Diag}(u)V_1V_2\text{Diag}(v)$ where $u=v=\mathbf{1}_n$, $V_1=a$ and $V_2 = b^T$.

\paragraph{Overall Computation.} Finally we are able to obtain a linear time algorithm with respect to the number of sample to compute the GW distance. Indeed, to summarize, we need  $\mathcal{O}(rr_{\ell}n)$ operations to compute $G^{(\ell)}$, $\mathcal{O}(r^2 n)$ operations to compute the factorization of $C^{(\ell)}$ from $G^{(\ell)}$, that is $U^{(\ell)}$ and $T^{(\ell)}$, $\mathcal{O}(rr_{\ell} n)$ operations to compute the low-rank factorization of the kernel, each iteration of the Sinkhorn algorithm can be performed in $\mathcal{O}(r_{\ell}n)$ algebraic operations thanks to the factorization of $C^{(\ell)}$ and finally computing the GW distance requires only  $\mathcal{O}(nr(r_{I-1}+r)+r^3)$ operations. Therefore the overall computation cost of the GW distance by Algorithm~(\ref{alg-lin-GW}) is $\mathcal{O}(nr( r_{\text{tot}}+Ir)+ \sum_{\ell=0}^{I-1} T_{\ell} n r_\ell + r^3)$ where $r_{\text{tot}}:=\sum_{\ell=0}^{I-1} r_{\ell}$, $T:=\sum_{\ell=0}^{I-1} T_{\ell}$ and  $T_{\ell}$ is the number of iterations of the Sinkhorn Algorithm~(\ref{alg-sink}) at iteration $\ell$ for a precision $\mu_{\ell}$.

Let us now show our main result on the approximation of the solution of Algorithm~(\ref{alg-mirror-descent}). In the following we denote by $\Vert\cdot\Vert$ the matrix norm defined as the maximum of the $\ell_2$-norm of its columns and $\tilde{\mathcal{O}}(.)$ means that we omits polylogarithmic factors w.r.t the constants of the problem.

\begin{thm}
\label{thm:rf-approx}
Let $I\geq 1$, $0<\delta\leq 1$ and $\tau\in(0,1)$. If for all $\ell\in\{0,..,I-1\}$
\begin{align*}
 r_{\ell}\in\Omega\left(\frac{\psi^2}{\mu_\ell^2}\log\left(\frac{n I}{\tau}\right)\right)
\end{align*}
where 
\begin{align*}
    \psi&:= 2^{d/2+1} \left(\frac{R_{0}^2}{4\varepsilon r W_0\left(R_0^2/\varepsilon r\right)}\right)^{d/2}\\
    R_{0}&:=\max\left(\Vert A\Vert_{\ell_\infty}\Vert D'\Vert_{\ell_1},\Vert A\Vert\right)\\
   \mu_\ell&:=\frac{\varepsilon \delta_\ell^2}{200\left[R + 1 +  \log\left(\frac{2\max(n,m)}{\delta_\ell^2}\right)\right]}\\
   \delta_\ell&:=\min\left(\frac{\delta}{2L I},\frac{\delta}{2L I(R/\varepsilon)^{I-(\ell+1)}}\right)\\
   L&:=\sup_{i,j,k,l}|D_{i,k}-D_{j,j}|^2 \text{\quad and \quad}  R:=4 \Vert D\Vert_{\text{op}}\Vert D'\Vert_{\text{op}}
\end{align*}
then the Gromov-Wasserstein Alg.~(\ref{alg-lin-GW}) with input  $(R_{\ell})_{ 0 \leq \ell\leq I-1}$, $(r_{\ell})_{ 0 \leq \ell\leq I-1}$ and $(\mu_{\ell})_{ 0 \leq \ell\leq I-1}$ outputs an approximation of the GW distance  $\widehat{\mathcal{E}}$ such that with a probability of at least $1-\tau$ we have:
\begin{align*}
    %\Vert P^{(I)} - Q^{(I)}\Vert_1&\leq \frac{\delta}{2L}\\
    |\mathcal{E}_{D,D'}(P^{(I)}) - \widehat{\mathcal{E}}|&\leq \delta.
\end{align*}
\end{thm}

\begin{rmq}
Note that with a probability of $1-\tau$, the total number of iterations of the Sinkhorn algorithm at iteration $\ell\in\{0,..,I-1\}$, is given by
$$T_\ell \in\widetilde{\mathcal{O}}\left(\mu_\ell^{-1}\varepsilon^{-1}R\right)$$.
\end{rmq}

% Let us now justify why the Assumption~(\ref{assump-low-rank}) of a low-rank factorization for the distance matrices $D$ and $D'$ is well suited in the problem of computing Gromov Wasserstein 
% distance.

% \paragraph{Square Euclidean Metric.} In the specific case where $D$ is a Square Euclidean distance matrix, it admits a low-rank decomposition. Indeed let $X:=[x_1,\dots,x_n]\in\mathbb{R}^{d\times n}$ where for all $i\in\{1,\dots,n\}$, $x_i\in\mathbb{R}^d$, and let $D:=(\Vert x_i-x_j\Vert_2^2)_{i,j}$. Then by denoting $p=[\Vert x_1\Vert_2^2,\dots,\Vert x_n\Vert_2^2]^T\in\mathbb{R}^n$ we can rewrite $D$ as the following:
% \begin{align*}
%     D=p\mathbf{1}_n^T + \mathbf{1}_np^T - 2 X^TX
% \end{align*}
% Therefore by denoting $A=[p,\mathbf{1}_n,-2X^T]\in\mathbb{R}^{n\times (d+2)}$ and $B^T=[\mathbf{1}_n,p,X^T]\in\mathbb{R}^{n\times (d+2)}$ we obtain that
% \begin{align*}
%     D=AB
% \end{align*}

% \paragraph{General Case: Distance Matrix.}
% In fact it is always possible to obtain an approximate low-rank factorization of a distance matrix. Indeed as $D$ is obtained from a metric, $D$ is therefore symmetric. Then by the Gershgorin circle theorem, on can estimate an upper bound of the biggest singular value by
% $$\sigma_D\leq \max_{i}\left(R_i:=\sum_{j}|D_{i,j}|\right).$$
% Computing the above upper bound of $\sigma_D$ requires $\mathcal{O}(n^2)$, but in fact we can obtain an upper bound in linear time by taking the advantage that it is a distance matrix. Indeed by the triangular inequality we have that for all $i\in \{1,\dots,n\}$,
% $$ R_i\leq R_1 + (n-1)\times D_{1,i} $$
% and therefore 
% $$\sigma_D\leq R_1 + (n-1) \max_{i}\left(D_{1,i}\right).$$
% Now remark that $D+\sigma_D \text{I}_n$ is a positive semi-definite matrix and applying a Nystrom method \todo{Pb: Nystrom depends on the effective dimension => Approx Musco for PSD matrix independent w.r.t the condition number: pb it does not admit a low rank factorisation as the matrix will be full rank.../ Otherwise check paper factorization distance matrix} leads to an efficient approximate low-rank factorization of $D+\sigma_D \text{I}_n$ 
% $$ D+\sigma_D\simeq \text{I}_n A_1A_1^T.$$
% Therefore we end up with an approximation $\tilde{D}$ of the matrix $D$ of the form 
% $$D\simeq \tilde{D}:=A_1A_1^T - \sigma_D \text{I}_n$$
% in $\mathcal{O}(n r+ r^3)$ algebraic operations.
% In fact even with distance matrices of this form we are able to apply our method to compute the GW distance in linear time with respect to the number of samples. Indeed the only requirement that we need to perform the iterations of the Algorithm~(\ref{alg-lin-GW}) in linear time is finally the cost function of the Sinkhorn algorithm admits a low-rank factorization which is still the case as we have at iteration $\ell$:
% \begin{align*}
% C^{(\ell)} & = - 4 \tilde{D} P^{(\ell)} \tilde{D'}\\
% &- 4 (A_1A_1^T - \sigma_D \text{I}_n) P^{(\ell)}  (B_1B_1^T - \sigma_{D '}\text{I}_n)\\
% & =  - 4A_1A_1^T P^{(\ell)} B_1B_1^T  - 4\sigma_D\sigma_{D '} P^{(\ell)}\\
% & + 4\sigma_D P^{(\ell)} B_1B_1^T + 4\sigma_{D '}A_1A_1^T P^{(\ell)}  
% \end{align*}
% But recall that $P^{(\ell)}$ admits a low-rank factorization of the form 
% \begin{align*}
% P^{(\ell)}&= Q^{(\ell)}R^{(\ell)} \quad \text{where}\\
% Q^{(\ell)}&:=\text{Diag}(u^{(\ell)}) V_1^{(\ell-1)} \\
% R^{(\ell)}&:=V^{(\ell-1)}_2 \text{Diag}(v^{(\ell)}).
% \end{align*}
% Therefore we obtain that:
% \begin{align*}
%     C^{(\ell)} &= - T^{(\ell)}U^{(\ell)} - 4\sigma_D\sigma_{D '} Q^{(\ell)}R^{(\ell)}\\
%     &+ 4\sigma_D Q^{(\ell)}R^{(\ell)}  B_1B_1^T + 4\sigma_{D '}A_1A_1^T Q^{(\ell)}R^{(\ell)}
% \end{align*}
% where
% \begin{align*}
%     T^{(\ell)} = 4A_1, \quad U^{(\ell)} =G^{(\ell)} B_1^{T}, \quad G^{(\ell)} = A_1^{T} P^{(\ell)} B_1
% \end{align*}
% and by denoting 
% \begin{align*}
%     T_2^{(\ell)}&:= - \sigma_D Q^{(\ell)}R^{(\ell)}  B_1\\
%     U_2^{(\ell)}&:=-\sigma_{D '} A_1^T Q^{(\ell)}R^{(\ell)}
% \end{align*}
%  we obtain that
% \begin{align*}
%      C^{(\ell)}&=- \tilde{T}^{(\ell)}\tilde{U}^{(\ell)} \text{\quad where}\\
%      \tilde{T}^{(\ell)}&:=[T^{(\ell)},2\sigma_D Q^{(\ell)},T_2^{(\ell)},4A_1]\in\mathbb{R}^{n\times (3r+r_{\ell})}\\
%      (\tilde{U}^{(\ell)})^T&:=[(U^{(\ell)})^T,2\sigma_{D'} (R^{(\ell)})^T,4B_1,(U_2^{(\ell)})^T]
% \end{align*}
% Therefore the overall computation cost for obtaining such factorization of the matrix $C^{(\ell)}$ at each iteration of the algorithm~(\ref{alg-lin-GW}) given the approximated distance matrices of $\tilde{D}$ and $\tilde{D'}$ is $\mathcal{O}(nr(r_{\ell}+r)+r^3)$. It worth noting that here we do not need to require the positivity of the factorization of $D$ and $D'$ when using a Nystrom method which was the main drawback when one wants to apply such technique to perform the Sinkhorn iterations.

% Finally computing $\mathcal{E}_{D,D'}(P^{(\ell)})$ can also be performed in linear time with respect to the number of samples as we have:
% \begin{align*}
% \langle \tilde{D}P^{(\ell)}\tilde{D'} ,P^{(\ell)}\rangle & = \text{Tr}((P^{(\ell)})^T A_1A_1^T P^{(\ell)} B_1B_1^T)\\
% &+  \text{Tr}((P^{(\ell)})^T 4\sigma_D\sigma_{D '} P^{(\ell)})\\
% &-  \text{Tr}((P^{(\ell)})^T\sigma_D P^{(\ell)} B_1B_1^T) \\ 
% & - \text{Tr}((P^{(\ell)})^T\sigma_{D '}A_1A_1^T P^{(\ell)})
% \end{align*}
% which can be written as the following:
% \begin{align*}
% \langle \tilde{D}P^{(\ell)}\tilde{D'} ,P^{(\ell)}\rangle & = \text{Tr}((G^{(\ell)}(G^{(\ell)})^T)\\
% &+ 4\sigma_D\sigma_{D '} \text{Tr}(( (Q^{(\ell)})^T Q^{(\ell)} R^{(\ell)} (R^{(\ell)})^T)\\
% & - \sigma_D \text{Tr}((P^{(\ell)}B_1)^T P^{(\ell)} B_1) \\ 
% & -  \sigma_{D '} \text{Tr}(A_1^T P^{(\ell)} (A_1^T P^{(\ell)})^T )
% \end{align*}
% But computing $Q^{(\ell)})^T Q^{(\ell)}\in\mathbb{R}^{r_{\ell}\times r_{\ell}}$, $R^{(\ell)} (R^{(\ell)})^T\in\mathbb{R}^{r_{\ell}\times r_{\ell}}$, $P^{(\ell)}B_1\in\mathbb{R}^{n\times r}$ and $A_1^T P^{(\ell)}\in\mathbb{R}^{r\times n}$ requires only $\mathcal{O}(nr_{\ell}(r_{\ell} + r))$.  Finally computing $\Vert P^{(\ell)}B_1 \Vert_2^2$ given $P^{(\ell)}B_1$ can be done in $\mathcal{O}(nr^2)$, and it the same for  $\Vert A_1^T P^{(\ell)} \Vert_2^2$. Therefore the overall computation cost to compute $\mathcal{E}_{D,D'}(P^{(\ell)})$ is $\mathcal{O}(n(r^2 + (r_{\ell})^2) + r^3)$.






==> not_include/sec4.tex <==
\section{Applications}




\todo{explain the stable version: when the gradient is taken with the constant + stable Sinkhorn !}
